Protecting the 'Stop Using My Data' Right through Blockchain-assisted Evidence Generation

In order to provide personalized services to users, Internet-based platforms collect and utilize user-generated behavioral data. Although the 'stop using my data' right should be a fundamental data right, which allows individuals to request their personal data to be no longer utilized by online platforms, the existing preventive data protection measures (e.g., cryptographic data elimination, differential privacy) are unfortunately not applicable. This work aims to develop the first Evidence Generation Framework for deterring post-acquisition data right violations. We formulated the 'stop using my data' problem, which captures a vantage facet of the multi-faceted notion of 'right to be forgotten'. We designed and implemented the first blockchain-assisted system to generate evidence for deterring the violations of the 'stop using my data' right. Our system employs a novel two-stage evidence generation protocol whose efficacy is ensured by a newly proposed Lemma. To validate our framework, we conducted a case study on recommendation systems with systematic evaluation experiments using two real-world datasets: the measured success rate exceeds 99%.

==> Old_Algorithm.tex <==
\section{Algorithm Design}

\subsection{Grey-box}
In a grey-box setting, the recommendation system utilizes the publicly available collaborative filtering algorithm. The detection system evaluates the recommendations generated by this algorithm using the same approach.

\begin{algorithm} [H]
\caption{Collaborate Filtering Algorithm}
    \begin{algorithmic}[1]
        \State \textbf{Input}: Similarity map $S$; Purchase history $\Vec{H_u}$; Number of recommendation $N$;
        \For{Each item $i$}
        \State Calculate $s_{u,i} = \sum_{j \in H_u} S(i,j)r_{u,j}$
        \EndFor
        \State Find the $N$ largest $s_u$ as $\Vec{s}_{u,N}$
        \State return $\Vec{s}_{u,N}$
    \end{algorithmic} 
\end{algorithm}

%  We provide a theoretical lower bound for the recommended content of a non-infringing system. Given that the recommendation before time $t$ is $\vec r_{acc^-}$ and the recommendation after time $t$ is $\vec r_{acc^+}$, we calculate the scores of $\vec r_{acc^-}$ and $\vec r_{acc^+}$ in the auxiliary dataset as $S_{aux}(\vec r_{acc^-})$ and $S_{aux}(\vec r_{acc^+})$.

% Based on the constraint of \ref{de:data similar}, we can get the range of the score in real dataset:

% $\Pr\left[(1-\theta)S_{aux}(\vec r_{acc^-})\leq S(\vec r_{acc^-})\leq (1+\theta)S_{aux}(\vec r_{acc^-})\right]\geq \gamma$

% $\Pr\left[(1-\theta)S_{aux}(\vec r_{acc^+})\leq S(\vec r_{acc^+})\leq (1+\theta)S_{aux}(\vec r_{acc^+})\right]\geq \gamma$

% So, the probability of $(1-\theta)S_{aux}(\vec r_{acc^+})<(1+\theta)S_{aux}(\vec r_{acc^-})$ should be less than $\gamma^2$.

% In practical datasets, obtaining an accurate value of $\gamma$ poses a challenge. Consequently, an approximation approach is adopted whereby the previous recommendation is utilized to predict $\gamma$.

\begin{algorithm} [H]
\caption{The proof generation v1}
    \begin{algorithmic}[1]
        %%%%%%% Get Trend
        \For{$\Vec{t_m} < t^-$ and $m < M$} \textcolor{blue}{\Comment{Calculate Trend}}
        \State  Calculate $S_{t_m}, \Vec{R}_{t_m}$ = \textbf{MPC($t_m$)}
        \State Calculate $\Vec{r}_{t_m}$ = \textbf{Recommendation($\Vec{H}_{t_m}$, $S_{t_m}$)}
        \EndFor
        %%%%%% Get Change
        \State  Calculate $S_{t^-}, \Vec{R}_{t^-}$ = \textbf{MPC($t^-$)} \textcolor{blue}{\Comment{Calculate Change}}
        \State Calculate $S_{t^+}, \Vec{R}_{t^+}$ = \textbf{MPC($t^+$)} 
        \State Calculate $\Vec{r}_{t^-}$ = \textbf{Recommendation($\Vec{H}_{t^-}$, $S_{t^-}$)}  
        \State Calculate $\Vec{r}_{t^+}$ = \textbf{Recommendation($\Vec{H}_{t^+}$, $S_{t^+}$)}
        %%%%%% Compare change and trend
        \For{$m<M$}
        \For{items $i$ in $\Vec{r}_{t_m}$}
        \For{items $u$ in $\Vec{r}_{t^-}$}
            \State Get $d_{t_m,ui}$ = $S_{t_m}(u, i)$
        \EndFor
        \EndFor
        \EndFor
        \For{items $i$ in $\Vec{r}_{acc^-}$}
        \For{item $u$ in $\Vec{r}_{t^-}$}
            \State Get $d_{t^-,ui}$ = $S_{t^-}(u, i)$
        \EndFor
        \EndFor
        \For{items $i$ in $\Vec{r}_{acc^+}$}
        \For{item $u$ in $\Vec{r}_{t^+}$}
        \State Get $d_{t^+,ui}$ = $S_{t^+}(u, i)$
        \EndFor
        \EndFor
        \For{$m<M$}
        \State Compare the distribution between $d_{t_m}$ and $d_{t^-}$
        \EndFor
        \State Compare the distribution between $d_{t^-}$ and $d_{t^+}$
    \end{algorithmic}
\end{algorithm}


\begin{algorithm} [H]
\caption{The proof generation v2}
    \begin{algorithmic}[1]
        %%%%%%% Get Trend
        \For{$\Vec{t_m} < t^-$ and $m < M$} \textcolor{blue}{\Comment{Calculate Trend}}
            \State  Calculate $S_{t_m}, \Vec{R}_{t_m}$ = \textbf{MPC($t_m$)}
            \State Get $s_{acc_m,ui}$ = $S_{t_m}(u, i)$
        \EndFor
        %%%%%%%Compare change
        \State  Calculate $S_{t^-}, \Vec{R}_{t^-}$ = \textbf{MPC($t^-$)}
        \State Calculate $S_{t^+}, \Vec{R}_{t^+}$ = \textbf{MPC($t^+$)} 
        % gradient part
        \For{items $i$ in $\Vec{r}_{acc^-}$ and $\Vec{r}_{acc^+}$}
        \For{item $u$ in $\Vec{H}_u^-$}
            \State Get $s_{acc^-,ui}$ = $S_{t^-}(u, i)$
            \State Get $s_{acc^+,ui}$ = $S_{t^+}(u, i)$
        \EndFor
        \EndFor
        \For{$m<M$}
            \State Compare the distribution of $s_{acc^-}$ and $s_{acc^+}$
        \EndFor
        \State Compare the distribution of $s_{acc^-}$ and $s_{acc^+}$
    \end{algorithmic}
\end{algorithm}

\subsection{Black-box}

==> Old_Dapp.tex <==
Due to the significant advancements in blockchain technology and its wide applications, {\em decentralized apps} (dApps) have been rapidly emerging. Evidently, The DApp industry saw a 50\% increase in daily active users from 1.58 million to 2.37 million in 2022 \cite{dappradar}.  Due to the following observations, decentralized apps are very different from {\em centralized} apps. (1) Centralized apps are typically owned by a singular entity, whereas ownership of DApps is decentralized. (2) DApps offer enhanced transparency, security, and accountability in transactions, while centralized apps lack these attributes. (3) Decentralized apps operate through a peer-to-peer network, which eliminates the need for intermediaries, unlike centralized apps that typically rely on intermediaries to facilitate transactions. 

No longer involving a central authority or trust, decentralized apps let several kinds of data rights become significantly more feasible to be protected through technical means. For example, the following motivating example illustrates the “Stop Use of My Data” right (``stop-use” right for short) in decentralized recommender systems.

{\bf Motivating example.} XXX (draw a figure to show a decentralized recommender system).
Note that the stop-use right is related to but not exactly the same as the right to have data erased.

==> Old_Data.tex <==
% \section{Case Study: Recommendation System \label{sec:case}}


%  The experimental section mainly aims to answer the following questions:

% {\bf Q1: How many data satisfy our probing situation?}

% {\bf Q2: What is the effectiveness of our detection system for data points and users that meet these criteria?}

% {\bf Q3: What is the impact of the relationship between the auxiliary dataset and the real dataset on the effectiveness?}  

% \subsection{Dataset}
% The datasets we collected and measured include Amazon's Electronic Product, Beauty, and Book datasets, the MovieLens Movie dataset, and Yahoo's ymusic dataset.

% The Amazon Dataset contains 82.83 million records and approximately 10 million items, rendering it impractical to calculate using the collaborative filtering algorithm. As a result, we split the whole dataset to several subdatasets categorized by item type, including electronic, beauty, and book \cite{ni2019justifying}. add: details of used datasets

% % https://nijianmo.github.io/amazon/index.html
% % https://nijianmo.github.io/amazon/index.html#subsets

% \subsection{Evaluation on probing situation}
% The majority of items have either zero or one associated items, indicating the sparsity of the dataset. This sparse characteristic makes the connection between data relatively simple (i.e., there are few associations between data), but also demonstrates that data with non-zero similarity have very close relationships with one another.

% The table \ref{tab:1} indicates that items with a similarity of one in the similarity map have been purchased very infrequently, posing a challenge in providing differential privacy protection for them. Eliminating these items from the dataset can significantly affect the recommendation system, particularly those strongly correlated with them, like those with similarity score one.

% \begin{table}[]
% \begin{tabular}{|l|cccccccc|} \hline 
% DataSet                                                      & \begin{tabular}[c]{@{}l@{}}Record \\ Number\end{tabular} & \begin{tabular}[c]{@{}l@{}}User \\ Number\end{tabular} & \begin{tabular}[c]{@{}l@{}}Item \\ Number\end{tabular} & Zero & One & Two & \begin{tabular}[c]{@{}l@{}}Three \\ to Nine \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Ten \\ or more\end{tabular}\\ \hline \hline
% \begin{tabular}[c]{@{}l@{}}Amazon\\ Digital Music\end{tabular} & 1584082 & 456992 & 840372 & 195506 & 80191
%  & 47461 & 136659 & 380555    \\ \hline
% \begin{tabular}[c]{@{}l@{}}Amazon\\ Beauty\end{tabular}  & 371345 & 32586 & 324038 & 28710 & 16806 & 12227 & 45198 & 221097 \\ \hline
% \begin{tabular}[c]{@{}l@{}}Amazon\\ Magazine\end{tabular}   & 89689 & 2428 & 72098 & 1906 & 1558 & 1373 & 6827 & 60434 \\ \hline
% \begin{tabular}[c]{@{}l@{}}MovieLens \\ Movie\end{tabular}  & 268130 & 2708 & 13156 & 1 & 0 & 0 & 30 & 13125 \\ \hline  
% \end{tabular}
% \caption{Statistical results of the total number of items and users as well as the number of items with non-zero similarity for each item, for example, zero represents the number of items whose non-zero similarity items is zero.}
% \label{tab:1}
% \end{table}


%  Our previous analysis of the dataset revealed a significant impact of item sparsity on detection results. Based on the contents of Table 1, we conducted the following analysis and scenario construction: 


% \begin{table}[H]
% \centering
% \begin{tabular}{|c|cccc|} 
% \hline
% \begin{tabular}[c] {@{}c@{}}The number of \\ `Being Alone' item\end{tabular} & Zero & One & Two & \begin{tabular}[c]{@{}c@{}}Three or\\ More\end{tabular} \\ \hline \hline
% Amazon-Beauty  &  10053  & 1191 & 858 & 0   \\ \hline
% Amazon-Book      & 3113 & 182& 186 & 19    \\ \hline
% Amazon-Electric     & 36335  &  4323   &  1358  &  0    \\ \hline
% Yahoo-Music                     &       &      &      &     \\ \hline
% iMovie-Movie     &  2708  & 0 & 0 & 0 \\ \hline
% \end{tabular}
% \caption{The number of users that have `being alone' items in different datasets.}
% \label{tab:2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|c|ccccc|}
% \hline
% & \begin{tabular}[c]{@{}l@{}}Amazon\\ Beauty\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Amazon\\ Book\end{tabular}  &  \begin{tabular}[c]{@{}l@{}}Amazon\\ Electronic\end{tabular}  &  \begin{tabular}[c]{@{}l@{}}Yahoo\\ Music\end{tabular}  & \begin{tabular}[c]{@{}l@{}}iMovie\\ Movie\end{tabular} \\ \hline
% \begin{tabular}[c] {@{}c@{}}The number of \\ `Couple'\end{tabular} & 1710 & 348 & 2716 &  &  0 \\ \hline
% \end{tabular}
% \caption{The number of `Couple' in different datasets.}
% \label{tab:3}
% \end{table}


% Table \ref{tab:2} displays the number of users who purchased items that had a limited number of non-zero items.

% We conducted tests on user-related data and organized the results into {\bf Table 3}. From the table, it is evident that the proportion of users who have purchased items with the `being alone' trait is xx, while the proportion of items with the 'being isolated' trait is xx.
% The aforementioned analysis leads to several conclusions: Firstly, the data in real systems exhibits sparsity, indicating a lack of correlation between a majority of items. Secondly, data sparsity implies that a significant portion of users possess highly sensitive data. As an illustration, in the XX dataset, a proportion of users' purchase histories contain isolated data. Lastly, the sensitivity of the data results in substantial changes in the recommendation content when the system exfiltrates some sensitive data. By detecting these changes, we can identify whether the system violates user privacy.

% Based on the analysis of the dataset discussed earlier, we can derive the following insights: 1) The sensitivity of an algorithm varies depending on the data, with the algorithm being highly sensitive to data that appears infrequently. 2) The sensitivity of a user's purchase history varies with the sparsity levels of the items, making users who have purchased sparser items more vulnerable to detection. 

% \subsection{Effectiveness of Evidence generation system}

% \subsection{The impact of auxiliary dataset}
% \section{Case Study: Recommendation System \label{sec:case}}

% \cite{shao2021survey}.

% \subsection{Collaborate Filtering}
% Collaborate filtering is a technique used in recommendation systems to provide users with personalized recommendations based on their historical preferences and behaviors \cite{sarwar2001item, linden2003amazon}. It works by analyzing the past interactions between users and items (movies, products, books, etc.) and then recommending new items to users based on the similarities between the users' preferences and behaviors. In item-based collaborative filtering, the algorithm calculates the similarity between items based on the ratings of users who have rated both items. A similarity map is constructed, which contains the pairwise similarity values between all items in the dataset. In this case study, we conducted an analysis using the collaborative filtering algorithm.


% \begin{algorithm} [h]
% \caption{Item-based Collaborate Filtering Algorithm}
%     \begin{algorithmic}[1]
%         \State \textbf{Input}: Item-user matrix $M$;Purchase history $\Vec{H_u}$; Number of recommendation $N$;
%         \For{Each item $i$ in $M$}
%         \State Calculate the cosine similarity $S_{i,j} = \frac{\mathbf{M_i} \cdot \mathbf{M_j}}{|\mathbf{M_i}| |\mathbf{M_j}|}$
%         \EndFor
%         \For{Each item $i$}
%         \State Calculate $s_{u,i} = \sum_{j \in H_u} S(i,j)r_{u,j}$
%         \EndFor
%         \State Find the $N$ largest $s_u$ as $\Vec{s}_{u,N}$
%         \State return $\Vec{s}_{u,N}$
%     \end{algorithmic} 
% \end{algorithm}

 
% The following experimental section mainly aims to answer the following questions:

% {\bf Q1: What is the proportion of data satisfying different protection levels in different datasets?}

% {\bf Q2: What is the effectiveness of our detection system for data points and users that meet these criteria?}

% {\bf Q3: What is the impact of the relationship between the auxiliary dataset and the real dataset on the effectiveness?}  

\begin{table*}[t]
\centering
\begin{tabular}{|l|cccccccc|} \hline 
DataSet                                                      & \begin{tabular}[c]{@{}l@{}}Record \\ Number\end{tabular} & \begin{tabular}[c]{@{}l@{}}User \\ Number\end{tabular} & \begin{tabular}[c]{@{}l@{}}Item \\ Number\end{tabular} & Zero & One & Two & \begin{tabular}[c]{@{}l@{}}Three \\ to Nine \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Ten \\ or more\end{tabular}\\ \hline \hline
\begin{tabular}[c]{@{}l@{}}Amazon\\ Digital Music\end{tabular} & 1584082 & 456992 & 840372 & 195506 & 80191
 & 47461 & 136659 & 380555    \\ \hline
\begin{tabular}[c]{@{}l@{}}Amazon\\ Beauty\end{tabular}  & 371345 & 32586 & 324038 & 28710 & 16806 & 12227 & 45198 & 221097 \\ \hline
% \begin{tabular}[c]{@{}l@{}}Amazon\\ Appliances\end{tabular}  & 371345 & 32586 & 324038 & 28710 & 16806 & 12227 & 45198 & 221097 \\ \hline
\begin{tabular}[c]{@{}l@{}}Amazon\\ Magazine\end{tabular}   & 89689 & 2428 & 72098 & 1906 & 1558 & 1373 & 6827 & 60434 \\ \hline
\begin{tabular}[c]{@{}l@{}}MovieLens \\ Movie\end{tabular}  & 268130 & 2708 & 13156 & 1 & 0 & 0 & 30 & 13125 \\ \hline  
\end{tabular}
\caption{Statistical results of the total number of items and users as well as the number of items with non-zero similarity for each item, for example, zero represents the number of items whose non-zero similarity items is zero.}
\label{tab:1}
\end{table*}

\subsection{Dataset Analysis}
The datasets we collected and measured include Amazon's Electronic Product, Beauty, and Book datasets, the MovieLens Movie dataset, and Yahoo's ymusic dataset.

The Amazon Dataset contains 82.83 million records and approximately 10 million items, rendering it impractical to calculate using the collaborative filtering algorithm. As a result, we split the whole dataset to several subdatasets categorized by item type, including electronic, beauty, and book \cite{ni2019justifying}. The MovieLens iMovie dataset is a popular dataset used in the field of recommender systems. It contains movie ratings provided by users of the MovieLens website, as well as movie metadata, including title, genre, and release year. With over 20 million ratings on over 27,000 movies, the dataset is commonly used for research on collaborative filtering algorithms and other recommendation system techniques \cite{harper2015movielens}.

% https://nijianmo.github.io/amazon/index.html
% https://nijianmo.github.io/amazon/index.html#subsets

\subsection{Evaluation on Probing Situation}


First, we analyzed the dataset, including the number of data entries, the number of items, the number of users, and the relationships between items. The majority of items have either zero or one associated items, indicating the sparsity of the dataset. This sparse characteristic makes the connection between data relatively simple (i.e., there are few associations between data), but also demonstrates that data with non-zero similarity have very close relationships with one another.

Based on the findings presented in Table \ref{tab:1}, it can be observed that almost all of Amazon's datasets exhibit sparse characteristics. In such cases, a large number of items with non-zero similarity is limited to only one. These items inherently meet characteristic `Being Isolated', and their corresponding `Outlier Output' value refers to the item with non-zero similarity. Concurrently, we observed that datasets such as MovieLen contain a sizable volume of reviews for each movie, resulting in high data correlation. Consequently, it is challenging to identify whether the system has exclusively relied on the output to determine data usage.



% \begin{table}[H]
% \centering
% \begin{tabular}{|c|cccc|} 
% \hline
% \begin{tabular}[c] {@{}c@{}}The number \\ of user\end{tabular} & One & Two & Three \\ \hline \hline
% Amazon-Beauty  &  10053  & 1191 & 858 & 0   \\ \hline
% Amazon-Book      & 3113 & 182& 186 & 19    \\ \hline
% Amazon-Electric     & 36335  &  4323   &  1358  &  0    \\ \hline
% Yahoo-Music                     &       &      &      &     \\ \hline
% iMovie-Movie     &  2708  & 0 & 0 & 0 \\ \hline
% \end{tabular}
% \caption{The number of users that have `being alone' items in different datasets.}
% \label{tab:2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|c|ccccc|}
% \hline
% & \begin{tabular}[c]{@{}l@{}}Amazon\\ Beauty\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Amazon\\ Book\end{tabular}  &  \begin{tabular}[c]{@{}l@{}}Amazon\\ Electronic\end{tabular}  &  \begin{tabular}[c]{@{}l@{}}Yahoo\\ Music\end{tabular}  & \begin{tabular}[c]{@{}l@{}}iMovie\\ Movie\end{tabular} \\ \hline
% \begin{tabular}[c] {@{}c@{}}The number of \\ `Couple'\end{tabular} & 1710 & 348 & 2716 &  &  0 \\ \hline
% \end{tabular}
% \caption{The number of `Couple' in different datasets.}
% \label{tab:3}
% \end{table}


% Table \ref{tab:2} displays the number of users who purchased items that had a limited number of non-zero items.

% We conducted tests on user-related data and organized the results into {\bf Table 3}. From the table, it is evident that the proportion of users who have purchased items with the `being alone' trait is xx, while the proportion of items with the 'being isolated' trait is xx.
% The aforementioned analysis leads to several conclusions: Firstly, the data in real systems exhibits sparsity, indicating a lack of correlation between a majority of items. Secondly, data sparsity implies that a significant portion of users possess highly sensitive data. As an illustration, in the XX dataset, a proportion of users' purchase histories contain isolated data. Lastly, the sensitivity of the data results in substantial changes in the recommendation content when the system exfiltrates some sensitive data. By detecting these changes, we can identify whether the system violates user privacy.

Based on the analysis of the dataset discussed earlier, we can derive the following insights: 1) The sensitivity of an algorithm varies depending on the data, with the algorithm being highly sensitive to data that appears infrequently. 2) The sensitivity of a user's purchase history varies with the sparsity levels of the items, making users who have purchased sparser items more vulnerable to detection. 

\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
Datset & All item & \begin{tabular}[c]{@{}l@{}}percentage\\ of user\end{tabular} & \begin{tabular}[c]{@{}l@{}}cluster\\ (aux)\end{tabular} & \begin{tabular}[c]{@{}l@{}}item in\\ cluster(aux)\end{tabular} & \begin{tabular}[c]{@{}l@{}}cluster\\ (real)\end{tabular} & \begin{tabular}[c]{@{}l@{}}item in\\ cluster(real)\end{tabular} & \begin{tabular}[c]{@{}l@{}}same\\ cluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}same\\ items\end{tabular} \\ \hline
Magazine & 72098         & 10\%   & 105      & 1651    & 91   & 2434    & 31  & 102  \\ \hline &     &     &    &       &      &     &    &    \\       &      &    &     &    &     &     &      &   \\ \hline 
\end{tabular}
\end{table}

\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=5cm]{cluster_real.jpg}
\caption{Cluster from real database.}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=5cm]{cluster_aux.jpg}
\caption{Cluster from auxiliary database.}
\end{minipage}
\end{figure}

\begin{figure*}[htbp]
    \centering  \includegraphics[width=5cm]{fig/probing.jpg}
    \caption{The effect of different probing times.}
    \label{fig:prob}
\end{figure*}

% \subsection{Effectiveness of Evidence generation system}

% \subsection{The impact of auxiliary dataset}



==> Old_Methods.tex <==
\section{Proposed Methods}

\subsection{Probing}
To facilitate evidence collection, we first analyzed the sensitivity of the data itself, that is, its impact on the system's output. We observed that some data are more sensitive than others. For example, in recommendation systems, there are items with very little associated data, causing their removal to significantly affect the output of the system. 
Here, we assume that we can input data arbitrarily to invoke the system's output, which is not feasible in real-world systems. 


For a given database and specified system, we define sensitivity with respect to the data in the database as follows:

\begin{definition}[Sensitivity from Dataset]
    For a data point $d_i$ in a given dataset $\mathcal{D}$, the output based on function is $O_i = \mathbb{F}_\mathcal{D}(d_i)$, we define $\frac{|O_i|}{|\mathcal{D}|}$ as the sensitivity of data $d_i$ for dataset $\mathcal{D}$ based on the function $\mathbb{F}$.
    
\end{definition}

From the definition of sensitivity, we know that as the sensitivity of the data with respect to the dataset decreases, its associated data becomes less and it becomes easier to affect the output. 
We provide the following definition for special data, i.e., data with extremely low sensitivity:

\begin{definition}[Being Alone]
For a data point $d_i$ in a given dataset $\mathcal{D}$, there is only one other item $d_j \in \mathcal{D}$ with $d_j = \mathbb{F}_\mathcal{D}(d_i)$, such that $d_i$ characterized as possessing the attribute `Being Alone'.
\end{definition}

\begin{definition}[Friend]
    A `friend' is defined as an items, namely item $d_i$, holds the `being alone' characteristic with $d_j$, we define $d_i$ is a friend with $d_j$.
\end{definition}
For all data that contain the attribute 'Being alone', they must necessarily be the friend of a certain data point. However, a data point may contain multiple 'friends', which is actually a one-to-many mapping relationship. Based on the above definition, we can deduce the following lemma:
\begin{lemma}
    For a data point with friends, when it is requested to be discontinued using, its friends will not appear in the output.
    \label{lemma:1}
\end{lemma}

For a specific user, their data sensitivity is not only related to the dataset and function, but also to their own historical data. Therefore, we define user-specific data sensitivity as follows:

\begin{definition}[Sensitivity from User]
    For a data point $d_i$ from user with previous dataset $D_u$ in a given dataset $\mathcal{D}$, the output based on function is $O_i = \mathbb{F}_\mathcal{D}(d_i)$ and $O_u = \mathbb{F}_\mathcal{D}(D_u)$. The union of two datasets is denoted as $D_{union}$, and the complement of dataset $D_i$ with respect to dataset $D_u$ is $D_{comp}$.we define $\frac{|D_{comp}|}{|D_{union}|}$ as the sensitivity of data $d_i$ for dataset $\mathcal{D}$ based on the function $\mathbb{F}$.
\end{definition}

For a user, we define special sensitive data as follows:

\begin{definition}[Being Isolated]
For any data point $d_i$ in a given dataset $\mathcal{D}$ and user $i$ with data $D_i = \{d_i, d_1,...d_k\}$, the output $O_d = \mathcal{F}_\mathbb{D}(D_i \setminus d_i)$ and $O_i = \mathcal{F}_\mathbb{D}(d_i)$ have no common data, such that $d_i$ characterized as possessing the attribute `Being Isolated'.
\end{definition}

\begin{lemma}
    For a user who holds a data $d_i$ satisfies `Being Isolated', if the data is requested to be stopped using, the data from $O_i$ should not appear in the output.
    \label{lemma:2}
\end{lemma}

\begin{definition}[Outlier output]
    For a data point $d_i$ in the output of a user, if this data point is only associated with one data point $d_j$ of the user, we refer to the data point $d_i$ as an outlier of the data point $d_j$.
\end{definition}

\begin{lemma}
    When a data point is requested to be stopped being used, its outliers will be removed in the output.
    \label{lemma:3}
\end{lemma}

For different data, their sensitivity to the entire database and users varies. The lower the sensitivity of the data, the greater the impact on the output because it is associated with very few data. Therefore, in the following sections, we classify these data and provide different levels of protection.

\subsection{Different Level Protection}

We categorize the data and users that can be protected into several levels starting from probing, namely completely protectable, relatively highly protectable, and not protectable.

{\bf Highly protectable}: For users who satisfy Lemma \ref{lemma:1}, Lemma \ref{lemma:2}, and Lemma \ref{lemma:3}, we can determine whether the system stops using this data point based on the changes in the output.

However, due to the unavailability of the real dataset, the precise values of $O_d = \mathcal{F}_\mathbb{D}(D_i)$ can only be derived from our auxiliary dataset, and may deviate from the actual output due to potential errors. The precise data we can obtain is only the output of the user's data at a specific time. So, the problem is how to address the information gap between auxiliary dataset and real dataset?


Drawing on insights \ref{insight:b} and \ref{insight:c}, we posit that the discrepancy between the auxiliary dataset and the real dataset is consistent. However, upon the removal of a user's designated data from the system, while the output based on the auxiliary dataset remains constant, the output derived from the real dataset will exhibit a variation. This variation can be quantified to discern whether the data has been successfully removed.

\begin{algorithm}[H]
\caption{Trend-Change Gap Evaluator}\label{alg:a}
\begin{algorithmic}[1]
\Function{Gap Evaluator}{$K$}\Comment{Evaluate the gap between two datasets}
\For{$i \gets 1$ to $K$}\Comment{Get trend between $t_1$ to $t_K$}
    \State $O_{aux,i} = \mathbb{F}_{\mathcal{D}_{aux}}(u_{t_i}), O_{real,i} = \mathbb{F}_{\mathcal{D}_{real}}(u_{t_i})$
    \State $d_i = \mathbb{D}(O_{aux,i}, O_{real,i})$
\EndFor
\State $O_{aux,0}^- = \mathbb{F}_{\mathcal{D}_{aux}}(u_{t_0}^-),  O_{real,0}^- = \mathbb{F}_{\mathcal{D}_{real}}(u_{t_0}^-)$ \Comment{Get the output before $t_0$}
\State $O_{aux,0}^+ = \mathbb{F}_{\mathcal{D}_{aux}}(u_{t_0}^+), O_{real,0}^+ = \mathbb{F}_{\mathcal{D}_{real}}(u_{t_0}^+)$ \Comment{Get the output after $t_0$}
\State $d_0^- = \mathbb{D}(O_{aux,0}^-, O_{real,0}^-), d_0^+ = \mathbb{D}(O_{aux,0}^+, O_{real,0}^+)$
\State Apply statistical methods to compare all $d$
\EndFunction
\end{algorithmic}
\end{algorithm}


In this algorithm, $\mathbb{F}$ represents the system function, $\mathbb{D}$ represents the distance function, such as the cosine distance, the Jaccard distance, and so on. In section \ref{sec:case}, we simulated and tested the algorithm based on the recommendation system to evaluate the probability of highly protectable data in the auxiliary dataset remaining protected in the real dataset.

Due to the information loss of the auxiliary dataset compared to the real dataset, there may be cases where the output based on the auxiliary dataset remains unchanged, but the output based on the real dataset changes. To address this issue, we introduce an auxiliary algorithm to measure the distance between the data and the target data. If the output data is closer to or unchanged compared to the target data than before the data was requested to be removed, we consider the system has not stopped using this data.

\begin{algorithm}
\caption{Data Distance Algorithm}\label{alg:b}
\begin{algorithmic}[1]
\Function{Distance Trend}{$d_0$}
\For{$p_i^-$ in $O_{aux}^-$, $p_i^+$ in $O_{aux}^+$}
    \State $d_{aux,i}^- = \mathbb{D}(d_0, p_i^-), d_{aux,i}^+ = \mathbb{D}(d_0, p_i^+)$
\EndFor
\For{$q_i^-$ in $O_{aux}^-$, $q_i^+$ in $O_{aux}^+$}
    \State $d_{real, i}^- = \mathbb{D}(d_0, q_i^-), d_{real, i}^+ = \mathbb{D}(d_0, q_i^+)$
\EndFor
\State Apply statistical methods to compare all $d$
\EndFunction
\end{algorithmic}
\end{algorithm}

{\bf Conditional Protectable}: For data a that does not satisfy Lemma \ref{lemma:1},\ref{lemma:2},\ref{lemma:3} but can cause differences in the output, we need to analyze the differences in the output to determine whether we can obtain evidence of its use. Combining Algorithm \ref{alg:a} and Algorithm \ref{alg:b}, we measured in the experiments in Section \ref{sec:case} how much the difference in d needs to be before we can protect the data with a certain probability.

{\bf Unprotectable}: For ordinary data, i.e., data $d_i$ where $O_i = \mathcal{F}_\mathbb{D}(d_i)$ is a subset of $O_d = \mathcal{F}_\mathbb{D}(D_i \setminus d_i)$, it is difficult to determine whether it has been used solely based on the output, because whether or not it is included, the system's output remains unchanged and the associated data of user data remains consistent. For this type of data, our system currently cannot protect its usage rights.

Due to the varying difficulty in protecting different types of data, the difficulty in protecting users who possess these data also varies. For example, in the Amazon recommendation system, data on items with low purchase frequency will have a greater impact on recommendations. For users, we can choose to test and supervise the sensitive data they possess to the system, even if there is a large amount of difficult-to-protect data, as long as there is a highly-protectable data, our system can monitor and extract evidence for them.

% $\bf Scenario~1$: The user $u$ holds a purchase history of $\{p_1,p_2, ...\}$ and the recommendation based on this purchase history is $\{r_1,r_2, ...\}$. The item $p_1$ holds `Being Alone' property in both auxiliary dataset and the real dataset and item $\{p_1,r_1\}$ is a `couple'. When user $u$ requests not to use purchase information of item $p_1$, if that user is still recommended item $r_1$, then the user's `stop use my data' rights have definitely been violated.

% $\bf Proof~1$: In accordance with the definition of `couple', the similarity score between two items $p_1$ and $r_1$ is exclusively non-zero. Consequently, item $r_1$ will be recommended only if item $p_1$ is present in the purchase history, and conversely, item $p_1$ will only be recommended in the presence of item $r_1$ within the purchase history.

% Scenario 1 is the most basic example and also includes our most fundamental idea: How to use this characteristic to protect user privacy for data that cannot be protected by differential privacy. Table 3, obtained from our analysis of the dataset, indicates that Scenario 1 is satisfied by relatively few data. Hence, it is necessary to relax the constraints and extend this scenario to encompass more general cases.

% {\bf Scenario~2}: The user $u$ holds a purchase history of $\{p_1,p_2, ...\}$ and the recommendation based on this purchase history is $\{r_1,r_2, ...\}$. The item $p_1$ holds `Being Alone' property and item $\{p_1,r_1\}$ is a `couple' in auxiliary dataset. In the real dataset, the item under consideration does not exhibit the characteristic of `Being Alone'. To define a set of items with a similarity score greater than zero, we denote this set as $S_i=\{r_1,i_1,i_2,...\}$. In this set, only $r_1$ has been recommended by the recommendation system, and the similarity between all other items in the set and the items in the user's purchase history is zero. Then the detection of this scenario is consistent with scenario 1.

% {\bf Proof~2}: Based on Assumption 1, the recommendation system always provides the most accurate recommendations. Therefore, regardless of whether the system violates the user's `stop use my data' rights, other items except $r_1$ in set $S_i$ will not be recommended. Therefore, this scenario can be transformed into Scenario 1.

% We conducted tests on the dataset with data ratios that satisfy scenarios 1 and 2, and the results were recorded in Table \ref{Tab:2}.

% The following discussion pertains to data that is relatively less `sensitive' and may exhibit a high degree of similarity or correlation with other data in the purchase history, thereby resulting in a larger set of associated items.

% {\bf Scenario~3}: The user $u$ holds a purchase history of $P=\{p_1,p_2, ...p_m\}$ and the recommendation based on this purchase history is $R=\{r_1,r_2, ...r_n\}$. We denote the set of items with a similarity score greater than zero with item $p_i$ as $I_i=\{i_1,i_2,...i_l\}$. In this set, $R_i=\{i_1,... i_r\}$ has been recommended by the recommendation system. There are other data points in the purchase history that exhibit non-zero similarity with the remaining items in the set $I_i$. 

% Upon removing the purchase history of $p_i$, it follows that the impact would only be felt by the items contained within set $I_i$, with a resultant reduction in their respective ratings. Define the score values of the individual elements belonging to set $I_i$, before and after the elimination of $p$, as $S_i^{-}=\{s_1^{-}, s_2^{-}, ...s_l^{-}\}$ and $S_i^{+}=\{s_1^{+}, s_2^{+}, ...s_l^{+}\}$, respectively. The relationship between the said scores can be described by the following expression:

% $s_j^{+}=s_j^{-}-s_{p,j}*r_p$, for all $i_j \in I_i$

% As a result of the observed decline in the ratings of items exclusively present in the set, it is possible to infer that the recommendation system has illicitly obtained access to user data when both the set and recommendation contain an increased number of items. Empirical evidence in Figure 1 further indicates that there is a probability of xx that the number of shared items between the set and recommendation will decrease.

==> Old_System.tex <==
\section{System Design}

$\bf Scenario~1$: The user $u$ holds a purchase history of $\{p_1,p_2, ...\}$ and the recommendation based on this purchase history is $\{r_1,r_2, ...\}$. The item $p_1$ holds `Being Alone' property in both auxiliary dataset and the real dataset and item $\{p_1,r_1\}$ is a `couple'. When user $u$ requests not to use purchase information of item $p_1$, if that user is still recommended item $r_1$, then the user's `stop use my data' rights have definitely been violated.

$\bf Proof~1$: In accordance with the definition of `couple', the similarity score between two items $p_1$ and $r_1$ is exclusively non-zero. Consequently, item $r_1$ will be recommended only if item $p_1$ is present in the purchase history, and conversely, item $p_1$ will only be recommended in the presence of item $r_1$ within the purchase history.

Scenario 1 is the most basic example and also includes our most fundamental idea: How to use this characteristic to protect user privacy for data that cannot be protected by differential privacy. Table 3, obtained from our analysis of the dataset, indicates that Scenario 1 is satisfied by relatively few data. Hence, it is necessary to relax the constraints and extend this scenario to encompass more general cases.

{\bf Scenario~2}: The user $u$ holds a purchase history of $\{p_1,p_2, ...\}$ and the recommendation based on this purchase history is $\{r_1,r_2, ...\}$. The item $p_1$ holds `Being Alone' property and item $\{p_1,r_1\}$ is a `couple' in auxiliary dataset. In the real dataset, the item under consideration does not exhibit the characteristic of `Being Alone'. To define a set of items with a similarity score greater than zero, we denote this set as $S_i=\{r_1,i_1,i_2,...\}$. In this set, only $r_1$ has been recommended by the recommendation system, and the similarity between all other items in the set and the items in the user's purchase history is zero. Then the detection of this scenario is consistent with scenario 1.

{\bf Proof~2}: Based on Assumption 1, the recommendation system always provides the most accurate recommendations. Therefore, regardless of whether the system violates the user's `stop use my data' rights, other items except $r_1$ in set $S_i$ will not be recommended. Therefore, this scenario can be transformed into Scenario 1.

We conducted tests on the dataset with data ratios that satisfy scenarios 1 and 2, and the results were recorded in Table \ref{Tab:2}.

The following discussion pertains to data that is relatively less `sensitive' and may exhibit a high degree of similarity or correlation with other data in the purchase history, thereby resulting in a larger set of associated items.

{\bf Scenario~3}: The user $u$ holds a purchase history of $P=\{p_1,p_2, ...p_m\}$ and the recommendation based on this purchase history is $R=\{r_1,r_2, ...r_n\}$. We denote the set of items with a similarity score greater than zero with item $p_i$ as $I_i=\{i_1,i_2,...i_l\}$. In this set, $R_i=\{i_1,... i_r\}$ has been recommended by the recommendation system. There are other data points in the purchase history that exhibit non-zero similarity with the remaining items in the set $I_i$. 

Upon removing the purchase history of $p_i$, it follows that the impact would only be felt by the items contained within set $I_i$, with a resultant reduction in their respective ratings. Define the score values of the individual elements belonging to set $I_i$, before and after the elimination of $p$, as $S_i^{-}=\{s_1^{-}, s_2^{-}, ...s_l^{-}\}$ and $S_i^{+}=\{s_1^{+}, s_2^{+}, ...s_l^{+}\}$, respectively. The relationship between the said scores can be described by the following expression:

$s_j^{+}=s_j^{-}-s_{p,j}*r_p$, for all $i_j \in I_i$

As a result of the observed decline in the ratings of items exclusively present in the set, it is possible to infer that the recommendation system has illicitly obtained access to user data when both the set and recommendation contain an increased number of items. Empirical evidence in Figure 1 further indicates that there is a probability of xx that the number of shared items between the set and recommendation will decrease.

\begin{definition}[Being Isolated]
    For an item $i$ and purchase history $P=\{p_1, p_2, ...\}$ in a given similarity map. Define $S_i=\{i_1,i_2,...\}$ as the item set that have non-zero similarity with items $i$. If all items in a set have a similarity of zero with other items in the purchase history, we define such an item $i$ have the `isolated' property.
\end{definition}

\begin{lemma}
When item $i$ has the `being isolated' trait, the applicable scenario is consistent with that of `Being Alone'.
\end{lemma}

We conducted tests on user-related data and organized the results into {\bf Table 3}. From the table, it is evident that the proportion of users who have purchased items with the 'being alone' trait is xx, while the proportion of items with the 'being isolated' trait is xx.
The aforementioned analysis leads to several conclusions: Firstly, the data in real systems exhibits sparsity, indicating a lack of correlation between a majority of items. Secondly, data sparsity implies that a significant portion of users possess highly sensitive data. As an illustration, in the XX dataset, a proportion of users' purchase histories contain isolated data. Lastly, the sensitivity of the data results in substantial changes in the recommendation content when the system exfiltrates some sensitive data. By detecting these changes, we can identify whether the system violates user privacy.

% Use auxiliary dataset, the recommendation before $t$, $\vec r_{t,b}$ and after $t$, $\vec r_{t,a}$ to judge whether the recommendation system steals the user's data.

